Sparse Visual Counterfactual Explanations in Image Space

Visual counterfactual explanations (VCEs) in image space are an important tool to understand decisions of image classifiers as they show under which changes of the image the decision of the classifier would change. Their generation in image space is challenging and requires robust models due to the problem of adversarial examples. Existing techniques to generate VCEs in image space suffer from spurious changes in the background. Our novel perturbation model for VCEs together with its efficient optimization via our novel Auto-Frank-Wolfe scheme yields sparse VCEs which lead to subtle changes specific for the target class. Moreover, we show that VCEs can be used to detect undesired behavior of ImageNet classifiers due to spurious features in the ImageNet dataset.

==> panels/afw_vs_apgd.tex <==
\begin{figure}[t]
\begin{minipage}[t]{.5\textwidth} 
     \centering
     \captionsetup{width=.9\linewidth}
     \begin{tabular}{ccc}
                   \hline
                   \multicolumn{1}{C{0.26\textwidth}}{$\;\;\;\;$ Original} & \multicolumn{1}{C{0.26\textwidth}}{AFW,$l_2$,\par$\epsilon=2.5$}&\multicolumn{1}{C{0.26\textwidth}}{APGD,$l_2$,\par$\epsilon=2.5$}\\
                   \hline
                   \multirow{4}{0.26\textwidth}{
                   \begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $\rightarrow$cat}
     \includegraphics[width=1\textwidth]{afw_vs_apgd/init_apgd_75_l2_2.5_GU_impr83_from_9_.png}
     \caption*{\tiny $\rightarrow$bird}
     \end{subfigure}
     }&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny \tiny $l_1$/$l_2$:$87.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny \tiny $l_1$/$l_2$:$82.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny \tiny $l_1$/$l_2$:$92.5$/$2.5$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny \tiny $l_1$/$l_2$:$92.2$/$2.5$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_wrong.png}
                    
                    \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}\\
                         
                             \hline

    \multirow{4}{0.26\textwidth}{
                   \begin{subfigure}{0.26\textwidth}\centering
     
    \caption*{\tiny $\rightarrow$car}
     \includegraphics[width=1\textwidth]{ablation_cifar_1_5/init_0.02l2_Francesco_small_radius_experimental20_from_9_.png}
     \caption*{\tiny $\rightarrow$truck}
     \end{subfigure}}&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny \tiny $l_1$/$l_2$:$94.8$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny \tiny $l_1$/$l_2$:$94.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny \tiny $l_1$/$l_2$:$91.8$/$2.5$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny \tiny $l_1$/$l_2$:$91.8$/$2.5$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_wrong.png}
                    
                    \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}\\ 
     \hline
     \end{tabular}
     \caption{\textbf{CIFAR10:} \label{fig:apgd_vs_afw_cifar10}$l_2$-VCEs at $\epsilon_2=2.5$ using AFW on the left and APGD on the right. Both achieve maximal confidence and most of the time the VCEs look similar but the top image with target ``cat'' shows that the non-convex problem of the VCEs can lead to quite distinct solutions.}
     \end{minipage}
     \begin{minipage}[t]{.5\textwidth}
     \centering
     \captionsetup{width=.9\linewidth}
     
     \begin{tabular}{ccc}
                   \hline
                   \multicolumn{1}{C{0.26\textwidth}}{$\;\;\;\;$ Original} & \multicolumn{1}{C{0.26\textwidth}}{AFW,$l_2$,\par$\epsilon=12$}&\multicolumn{1}{C{0.26\textwidth}}{APGD,$l_2$,\par$\epsilon=12$}\\
                   \hline
    \multirow{4}{0.26\textwidth}{
     \begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $\rightarrow$dung beetle}
     \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/init_afw_75_12_l2_Madry_l2_ep394_from_30.png}
     \caption*{\tiny $\rightarrow$tiger beetle}
     \end{subfigure}}&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $l_1$/$l_2$:$2817.6$\\/$11.8$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $l_1$/$l_2$:$2872.4$\\/$12.0$,
     $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny $l_1$/$l_2$:$2706.8$\\/$11.9$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny $l_1$/$l_2$:$2793.7$\\/$12.0$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30wrong.png}
                    
                    \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}\\
                         \hline
                         \multirow{4}{0.26\textwidth}{
                         \begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $\rightarrow$cauliflower}
     \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/init_afw_75_12_l2_Madry_l2_ep337_from_93.png}
     \caption*{\tiny $\rightarrow$head cabbage}
     \end{subfigure}}
     &\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $l_1$/$l_2$:$2978.4$\\/$11.9$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
     
     \caption*{\tiny $l_1$/$l_2$:$3020.3$\\/$12.0$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny $l_1$/$l_2$:$3477.8$\\/$11.9$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                    
                    \caption*{\tiny $l_1$/$l_2$:$3491.7$\\/$12.0$, $p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93wrong.png}
                    
                    \end{subfigure}\\&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.26\textwidth}\centering
                         \includegraphics[width=1\textwidth]{afw_vs_apgd_imagenet/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}\\ 
     \hline
     \end{tabular}
     \caption{\textbf{ImageNet:} \label{fig:apgd_vs_afw_imagenet}$l_2$-VCEs at $\epsilon_2=12$ using AFW on the left and APGD on the right. Both achieve maximal confidence and here the differences are even smaller than for CIFAR10.}
     \end{minipage}
     \end{figure}
            

==> panels/diversificatin.tex <==
\begin{figure}[hbtp!]
    
     \centering
     \begin{tabular}{cccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.115\textwidth}}{pVCE:$1e4$}&\multicolumn{1}{C{.115\textwidth}}{pVCE:$2e4$}&\multicolumn{1}{C{.115\textwidth}}{pVCE:$3e4$}\\
                   \hline
                   
                  
     \begin{subfigure}{0.115\textwidth}\centering  
     \caption*{$\rightarrow$frog,\\ $\rightarrow$:plane}
     \includegraphics[width=1\textwidth]{diversity/init_apgd19_from_6_.png}
     \end{subfigure}&
     \begin{subfigure}{0.115\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.32$, $p_e$:$1.00$}
     \includegraphics[width=1\textwidth]{diversity/PSGLA__1e4__prior_pgd19_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.115\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.32$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity/PSGLA__2e4__prior_pgd19_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.115\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.32$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity/PSGLA__3e4__prior_pgd19_from_6_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.115\textwidth}\centering
                
                \caption*{$l_2$:$5.0$, \\$p_i$:$0.19$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity/PSGLA__1e4__prior_pgd19_from_6_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.115\textwidth}\centering
                
                \caption*{$l_2$:$5.0$, \\$p_i$:$0.19$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity/PSGLA__2e4__prior_pgd19_from_6_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.115\textwidth}\centering
                
                \caption*{$l_2$:$5.0$, \\$p_i$:$0.19$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity/PSGLA__3e4__prior_pgd19_from_6_wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
    
     
    
   \centering
  \begin{tabular}{c|c|c|c}
    
    \backslashbox{Model}{FID$\downarrow$/MMPD$\uparrow$} & 1e4 & 2e4 & 3e4\\
    \hline
    
    PALMC & 19/NA &  18.5/3.9 & \cellcolor{green!25} 18.4/4.1  \\
    \hline
  \end{tabular}
  
  
     \caption{\label{fig:prior_diversity_bigger_radius}VCEs generated using PALMC with different seeds. Both qualitatively and quantitatively one can observe increasing diversity of pVCEs with big enough radius. Here MMPD stands for mean maximal pairwise distance between images across seeds.}
     \end{figure}
    

==> panels/failure_granny.tex <==
\begin{figure}[p!]
     
     \end{figure}


==> panels/fw_ODI_varying_seeds.tex <==
\begin{table}[hbt!]
     
     \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{ODI:$1e4$}&\multicolumn{1}{C{.12\textwidth}}{ODI:$2e4$}&\multicolumn{1}{C{.12\textwidth}}{ODI:$3e4$}&\multicolumn{1}{C{.12\textwidth}}{ODI:$4e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$1e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$2e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$3e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$4e4$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:frog,\\ \textbf{s}:cat}
     \includegraphics[width=1\textwidth]{diversity_ODI/init_ODI10_from_3_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase10_from_3_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$5.0$, \\$p_i$:$0.13$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase10_from_3_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase10_from_3_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase10_from_3_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.9$, \\$p_i$:$0.87$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase10_from_3_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase10_from_3_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:car,\\ \textbf{s}:truck}
     \includegraphics[width=1\textwidth]{diversity_ODI/init_ODI20_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$4.9$, \\$p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase20_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.7$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.7$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.7$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.7$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.8$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.8$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.8$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$4.8$, \\$p_i$:$0.83$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase20_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__ODI20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__ODI20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__ODI20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__ODI20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__iter_increase20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__iter_increase20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__iter_increase20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__iter_increase20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
       
        \begin{adjustbox}{width=1\columnwidth,center}
   \centering
  \begin{tabular}{c|c|c|c|c|c|c}
    
    \backslashbox{Type}{MMPD$\uparrow$} & 2 & 5 & 10 & 40 & 80 & 160\\
    \hline
    ODI & 5.6 & 7.8 & 9.2 & 11.7 & 11.8 & \cellcolor{green!25} 13.4 \\
    iters & 5.6 & 6 & 6.1 & 5.6 & 5.6 & 5.3\\
    \hline
  \end{tabular}
  \end{adjustbox}
  
       \caption{\label{tab:fw-cifar10-diversity}FW constrained to $l^{1.2}, l^{1.5}, l^2$ balls vs. PGD constrained to $l^2$ ball of a fixed radius.}
     \end{table}
   
  
  
     
     
     \begin{table}[hbt!]
      
      \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{ODI:$1e4$}&\multicolumn{1}{C{.12\textwidth}}{ODI:$2e4$}&\multicolumn{1}{C{.12\textwidth}}{ODI:$3e4$}&\multicolumn{1}{C{.12\textwidth}}{ODI:$4e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$1e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$2e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$3e4$}&\multicolumn{1}{C{.12\textwidth}}{iters:$4e4$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:submarine, p,\\ \textbf{s}:speedboat}
     \includegraphics[width=1\textwidth]{diversity_ODI/init_100042_from_62.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.8$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.5$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.5$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.8$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.8$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.5$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.5$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300042_from_62correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$24.8$, \\$p_i$:$0.08$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400042_from_62correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400042_from_62correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.4$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.7$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.8$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.4$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.4$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.7$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.8$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300042_from_62wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$24.4$, \\$p_i$:$0.08$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400042_from_62wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400042_from_62wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:koala, koala,\\ \textbf{s}:pot, flowerp}
     \includegraphics[width=1\textwidth]{diversity_ODI/init_100097_from_73.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.3$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.5$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.4$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.3$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.3$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.5$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.4$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300097_from_73correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$22.3$, \\$p_i$:$0.11$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400097_from_73correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400097_from_73correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.2$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.1$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.3$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.2$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.2$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.1$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.3$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300097_from_73wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.2$, \\$p_i$:$0.11$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400097_from_73wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400097_from_73wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:barometer,\\ \textbf{s}:bassoon}
     \includegraphics[width=1\textwidth]{diversity_ODI/init_100096_from_44.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.3$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.1$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.0$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.3$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.3$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.1$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.0$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300096_from_44correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_2$:$21.3$, \\$p_i$:$0.01$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400096_from_44correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400096_from_44correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300096_from_44wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_2$:$23.4$, \\$p_i$:$0.01$, $p_e$:$1.00$:$1.00$}
                \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400096_from_44wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__1e4__100096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__2e4__200096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__3e4__300096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/ODI__4e4__400096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__1e4__100096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__2e4__200096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__3e4__300096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{diversity_ODI/iter_increase__4e4__400096_from_44wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     \begin{adjustbox}{width=1\columnwidth,center}
   \centering
  \begin{tabular}{c|c|c|c|c|c|c}
    
    \backslashbox{Type}{MMPD$\uparrow$} & 2 & 5 & 10 & 40 & 80 & 160\\
    \hline
    ODI & 72.2 & 75.5 & 82.6 & 86.5 & 87.1 &\cellcolor{green!25} 89.1 \\
    iters & 69.6 & 68.8 & 69.7 & 71.7 & 75.5 & 78.8 \\
    \hline
  \end{tabular}
  \end{adjustbox}
  
     \caption{\label{tab:fw-in1k-diversity}FW constrained to $l^{1.2}, l^{1.5}, l^2$ balls vs. PGD constrained to $l^2$ ball of a fixed radius.}
     \end{table}
            

==> panels/fw_pgd_varying_radii.tex <==
\begin{table}[hbt!]
     
     \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_1    :20$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:6$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:2.5}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:2.5}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:cat,\\ \textbf{s}:bird}
     \includegraphics[width=1\textwidth]{afw/init_intersection_1.2_12.5_GU_impr83_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.4$, $p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$48.1$/$2.4$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$87.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$82.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.3$, $p_e$:$0.87$}
                \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$53.6$/$2.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$92.5$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$92.2$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:car,\\ \textbf{s}:truck}
     \includegraphics[width=1\textwidth]{afw/init_intersection_1.2_12.5_GU_impr20_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$1.8$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$55.7$/$2.2$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$94.8$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$94.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$52.3$/$2.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.8$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.8$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:plane,\\ \textbf{s}:deer}
     \includegraphics[width=1\textwidth]{afw/init_intersection_1.2_12.5_GU_impr92_from_8_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.9$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$47.2$/$2.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.7$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.4$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$47.7$/$2.4$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$86.7$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$87.1$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
       
        \begin{adjustbox}{width=1\columnwidth,center}
   \centering
  \begin{tabular}{c|c|c|c|c}
    
    \backslashbox{Model}{FID(ID/OD)$\downarrow$} & APGD,$l_1$:$20$ & FW,$l_{1.5}$:$6$ & FW,$l_2$:$2.5$ & APGD,$l_2$:$2.5$\\
    \hline
    GU-extra & 23.1/71.4 & 9.1/52.5 & 14.2/53.8 & 14.8/54.2 \\
    GU-extra\_ep1 & 6.1/52.7 &  \cellcolor{green!25} 6.6/43.4 & 9.9/41.2 & 10.1/41.2 \\
    \hline
  \end{tabular}
  \end{adjustbox}
  
       \caption{\label{tab:l1.5_FID_all_CIFAR10}FW constrained to $l^{1.2}, l^{1.5}, l^2$ balls vs. PGD constrained to $l^2$ ball of a fixed radius.}
     \end{table}
   
  
  
     
     
     \begin{table}[hbt!]
      
      
      \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_1:400$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:50$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:12}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:12}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:cauliflower,\\ \textbf{s}:head cabbag}
     \includegraphics[width=1\textwidth]{afw_IN1k/init_afw_75_12_l2_Madry_l2_ep337_from_93.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$10.3$, $p_e$:$0.75$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1476.0$/$10.1$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2978.4$/$11.9$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3020.3$/$12.0$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$11.2$, $p_e$:$0.85$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1710.2$/$9.5$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3477.8$/$11.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3491.7$/$12.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:reflex came,\\ \textbf{s}:red wine}
     \includegraphics[width=1\textwidth]{afw_IN1k/init_afw_75_12_l2_Madry_l2_ep372_from_96.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$13.9$, $p_e$:$0.39$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1335.8$/$11.0$, $p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2877.7$/$11.9$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2889.7$/$12.0$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$14.9$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1541.0$/$10.3$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3207.1$/$11.8$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3228.4$/$12.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:dung beetle,\\ \textbf{s}:tiger beetl}
     \includegraphics[width=1\textwidth]{afw_IN1k/init_afw_75_12_l2_Madry_l2_ep394_from_30.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$11.4$, $p_e$:$0.87$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1381.0$/$10.6$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2817.6$/$11.8$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2845.6$/$12.0$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$11.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1263.1$/$11.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2706.8$/$11.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2793.7$/$12.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_IN1k/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     
     \begin{adjustbox}{width=1\columnwidth,center}
   \centering
  \begin{tabular}{c|c|c|c|c}
    
    \backslashbox{Model}{FID(ID/OD)$\downarrow$} & APGD,$l_1$:$400$ & FW,$l_{1.5}$:$50$ & FW,$l_2$:$12$ & APGD,$l_2$:$12$\\
    \hline
    Madry-l2 & 9.2/41.6 & 4.6/24.3 & 4.6/22.5 & 4.9/22.8 \\
    Madry-l2\_ep3 & 6/35.7 &  \cellcolor{green!25} 3.6/22.6 & 4.1/22.7 & 4.3/23.1 \\
    \hline
  \end{tabular}
  \end{adjustbox}
  
     \caption{\label{tab:l1.5_FID_all_IN1k}FW constrained to $l^{1.2}, l^{1.5}, l^2$ balls vs. PGD constrained to $l^2$ ball of a fixed radius.}
     \end{table}
            

==> panels/fw_vs_pgd.tex <==

 
 
 \begin{figure}[!htbp]
 \centering
 \hspace*{-4em}
 \begin{subfigure}{.45\textwidth}
\centering
\vspace*{1.3em}
\includegraphics[height=0.95\linewidth, width=0.9\linewidth]{images/FW_motivation_CIFAR10/hist_pgd_vs_inv_3.png}
\end{subfigure} 
 \begin{subfigure}{.45\textwidth}   
 \captionsetup[subfigure]{font=tiny,labelfont=tiny}
\centering
\begin{adjustbox}{width=1.2\linewidth}
\fontsize{5}{5}\selectfont
 \begin{tabular}{ccccc}
 \hline
 \multicolumn{1}{c}{Orig.} &
 \multicolumn{1}{C{.16\textwidth}}{PM} &
 \multicolumn{1}{c}{FW} &
 \multicolumn{1}{C{.16\textwidth}}{PGD}\\
 \hline
 \begin{subfigure}{0.12\textwidth}\centering
 
 \allowdisplaybreaks
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 bird:$0.3$, \\
 deer:$0.7$}}}
 \vspace*{0.3em}
 \includegraphics[width=1\textwidth]{FW_motivation_CIFAR10/76_bird:start=0.27762,end=1.0_l_1: 150.37, l_2: 3.73, l_inf: 0.36, LPIPS: 0.30_first}
 
 \end{subfigure}
 &
 \begin{subfigure}{0.12\textwidth}\centering
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 bird:$1$, $l_2$:$2.99$
 }}}
 \vspace*{0.1em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_CIFAR10/pm_76_from_deer_to_bird_start=0.27640,end=1.00000_l_0_3072.0,l_1_122.16,l_2_2.99,l_inf_0.35,LPIPS_0.55_last.png}
 
 \end{subfigure}
&
 \begin{subfigure}{0.12\textwidth}\centering
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 bird:$1$, $l_2$:$4.22$}}}
 \vspace*{0.1em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_CIFAR10/fw_76_from_deer_to_bird_start=0.27640,end=1.00000_l_0_3072.0,l_1_179.17,l_2_4.22,l_inf_0.36,LPIPS_0.31_last.png}
 
 \end{subfigure}
 &
 \begin{subfigure}{0.12\textwidth}\centering
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 bird:$1$, $l_2$:$5.00$}
 }}
 \vspace*{0.1em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_CIFAR10/pgd_76_from_deer_to_bird_start=0.27640,end=1.00000_l_0_3072.0,l_1_211.80,l_2_5.00,l_inf_0.40,LPIPS_0.34_last.png}
 
 \end{subfigure}\\
 
 
 \hline
 \begin{subfigure}{0.12\textwidth}\centering
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 mortar:$0.1$, chest:$0.5$}
 }}
 \vspace*{0.3em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_imagenet1000/24_from_chest_to_mortar_start=0.07921,end=0.99921_l_0_150522.0,l_1_3043.16,l_2_12.00,l_inf_0.34,LPIPS_0.28_first.png}
 
 \end{subfigure}& 
 \begin{subfigure}{0.12\textwidth}\centering
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 mortar:$1$, $l_2$:$9.89$}
 }}
 \vspace*{0.1em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_imagenet1000/pm_l2ep3_24_from_chest_to_mortar_start=0.07921,end=0.99560_l_0_150522.0,l_1_2429.40,l_2_9.89,l_inf_0.29,LPIPS_0.26_last.png}
 
 \end{subfigure}&
 \begin{subfigure}{0.12\textwidth}\centering
 
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 mortar:$1$, $l_2$:$11.95$}
 }}
 \vspace*{0.1em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_imagenet1000/fw_l2ep3_24_from_chest_to_mortar_start=0.07921,end=0.99898_l_0_150522.0,l_1_3046.51,l_2_11.95,l_inf_0.34,LPIPS_0.28_last.png}
 
 \end{subfigure}&
 \begin{subfigure}{0.12\textwidth}
 \centering
 
 \caption*{
 \scalebox{0.7}{\parbox{0.5cm}{
 mortar:$1$, $l_2$:$12.00$}
 }}
 \vspace*{0.1em}
 \includegraphics[width=1\textwidth]{images/FW_motivation_imagenet1000/pgd_l2ep3_24_from_chest_to_mortar_start=0.07921,end=0.99921_l_0_150522.0,l_1_3043.16,l_2_12.00,l_inf_0.34,LPIPS_0.28_last.png}
 
 \end{subfigure}
 \\
 \hline
 \end{tabular}

\end{adjustbox}
 
 \end{subfigure}
  \vspace*{-1em}
  \caption{\label{tab:FW_motivation}Choosing a radius $\epsilon$ is not trivial - here on the right it is shown, how for a fixed radius $\epsilon=5, \epsilon=12$ of $B_2(x^0, \epsilon)$ respectively for CIFAR10, ImageNet-1000 we find VCEs in interior using PM and FW.}
 \end{figure}
 


==> panels/imagenet_boats_counterfactual.tex <==
\begin{figure}[hbt!]
     \centering
     \small
     \begin{tabular}{cccc}
     \hline
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=100$}\\
     \hline
       
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{lifeboat: 0.51}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/original.png}
     \end{subfigure} &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$gondola: 0.97}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_0_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$gondola: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_0_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$gondola: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_0_radius_2.png}
     \end{subfigure} \\
     
      
      &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$fireboat: 0.57}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_1_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$fireboat: 0.98}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_1_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$fireboat: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_1_radius_2.png}
     \end{subfigure} \\

      
     &     
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$speedboat: 0.15}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_2_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$speedboat: 0.60}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_2_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$speedboat: 0.91}
     \includegraphics[width=1\textwidth]{images/imagenet_boats/target_2_radius_2.png}
     \end{subfigure} \\


     \end{tabular}
      \caption{\label{tab:imagent_valley}$l_{1.5}$-VCEs for Madry\cite{robustness}+FT with varying radii for a correctly classified image of class ``lifeboat'' for the target classes ``gondola'', ``fireboat'' and ``speedboat'' (same wordnet category ``boat'').
    
    }
     \end{figure}


==> panels/imagenet_food_counterfactual.tex <==
\begin{figure}[hbt!]
     \centering
     \small
     \begin{tabular}{cccc}
     \hline
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=100$}\\
     \hline
       
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{potpie: 0.68}
     \includegraphics[width=1\textwidth]{images/imagenet_food/original.png}
     \end{subfigure} &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$potpie: 0.97}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_2_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$potpie: 0.99}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_2_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$potpie: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_2_radius_2.png}
     \end{subfigure} \\
     
      
      &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$pizza: 0.11}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_1_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$pizza: 0.51}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_1_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$pizza: 0.86}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_1_radius_2.png}
     \end{subfigure} \\

      
     &     
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$cheeseburger: 0.61}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_3_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$cheeseburger: 0.96}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_3_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$cheeseburger: 0.99}
     \includegraphics[width=1\textwidth]{images/imagenet_food/target_3_radius_2.png}
     \end{subfigure} \\


     \end{tabular}
      \caption{\label{tab:imagent_valley}$l_{1.5}$-VCEs for Madry\cite{robustness}+FT with varying radii for a correctly classified image of class ``potpie'' for the target classes ``potpie'', ``pizza'' and ``cheeseburger'' (same wordnet category ``dish'').
    
    }
     \end{figure}


==> panels/imagenet_temple_counterfactual.tex <==
\begin{figure}[hbt!]
     \centering
     \small
     \begin{tabular}{cccc}
     \hline
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=100$}\\
     \hline
       
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{trium. arch: 0.53}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/original.png}
     \end{subfigure} &
     
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$trium. arch: 0.99}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_0_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$trium. arch: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_0_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$trium. arch: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_0_radius_2.png}
     \end{subfigure} \\
     
     &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$brass: 0.10}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_2_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$brass: 0.59}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_2_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$brass: 0.98}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_2_radius_2.png}
     \end{subfigure} \\
     
      
      &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$megalith: 0.62}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_1_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$megalith: 0.96}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_1_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$megalith: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_1_radius_2.png}
     \end{subfigure} \\

      
 



     \end{tabular}
      \caption{\label{tab:imagent_valley}$l_{1.5}$-VCEs for Madry\cite{robustness}+FT with varying radii for a correctly classified image of class ``triumphal arch'' for the target classes ``triumphal arch'', ``brass'' and ``megalith'' (same wordnet category ``memorial monument'').
    
    }
     \end{figure}


==> panels/imagenet_vces/amphibian_axolotl.tex <==
\begin{figure}[hbt!]
     \centering
     \begin{tabular}{cccc}
     \hline
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=100$}\\
     \hline
       
    
       
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{axolotl: 0.18}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/original.png}
     \end{subfigure}
     &     
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ axolotl: 0.99}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_5_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ axolotl: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_5_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ axolotl: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_5_radius_2.png}
     \end{subfigure} \\
     
    
      &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ fire salamander: 0.47}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_1_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ fire salamander: 0.95}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_1_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ fire salamander: 0.99}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_1_radius_2.png}
     \end{subfigure} \\
     
    
     &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ common newt: 0.47}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_2_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ common newt: 0.91}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_2_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ common newt: 0.98}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_2_radius_2.png}
     \end{subfigure} \\
     
    
     &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ eft: 0.29}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_3_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ eft: 0.93}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_3_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ eft: 0.99}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_3_radius_2.png}
     \end{subfigure} \\


    
      &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ tailed frog: 0.08}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_0_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ tailed frog: 0.39}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_0_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ tailed frog: 0.73}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/amphibian_axolotl/target_0_radius_0.png}
     \end{subfigure} \\


     \end{tabular}
      \caption{}
     \end{figure}


==> panels/imagenet_vces/dish.tex <==
\begin{figure}[ht]
     \centering
     \begin{tabular}{cccc}
     \hline
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=100$}\\
     \hline
       
    
       
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{pizza: 0.11}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/original.png}
     \end{subfigure} &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ potpie: 0.57}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_2_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ potpie: 0.86}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_2_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ potpie: 0.96}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_2_radius_2.png}
     \end{subfigure} \\
     
      
     &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ pizza: 0.92}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_1_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ pizza: 0.98}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_1_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ pizza: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_1_radius_2.png}
     \end{subfigure} \\

      
     &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ cheesburger: 0.80}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_5_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ cheesburger: 0.97}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_5_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ cheesburger: 1.00}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/dish/target_5_radius_2.png}
     \end{subfigure} \\


     \end{tabular}
      \caption{}
     \end{figure}


==> panels/imagenet_vces/failure_combined.tex <==
\begin{figure*}[htb!]
     \centering
     
     
     
     
    \begin{tabular}{cccc | cccc}
     \hline
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}|}{$\epsilon=100$} &
     \multicolumn{1}{c}{Original} & \multicolumn{1}{C{.115\textwidth}}{$l_{1.5}$, $\epsilon=50$} & 
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=75$} &
     \multicolumn{1}{C{.115\textwidth}}{$\epsilon=100$}
     \\
     \hline
     
      \begin{subfigure}{0.115\textwidth}\centering
     \caption*{tabby: 0.08}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/domestic_cat_tabbus/original.png}
     \end{subfigure} &
     
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$  tiger cat: 0.71}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/domestic_cat_tabbus/target_1_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$  tiger cat: 0.88}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/domestic_cat_tabbus/target_1_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$  tiger cat: 0.95}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/domestic_cat_tabbus/target_1_radius_2.png}
     \end{subfigure} &

     
\\
     
    
       &
     
     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ persian cat: 0.63}
     \includegraphics[width=1\textwidth]{images/imagenet_appendix_examples/domestic_cat_tabbus/target_2_radius_0.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ persian cat: 0.89}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_2_radius_1.png}
     \end{subfigure} &

     \begin{subfigure}{0.115\textwidth}\centering
     \caption*{$\rightarrow$ persian cat: 0.96}
     \includegraphics[width=1\textwidth]{images/imagenet_temple/target_2_radius_2.png}
     \end{subfigure} &


    
\\
    
    
    \hline
    \multicolumn{4}{c|}{WordNet: domestic cat - GT class: tabby}
    &
    \multicolumn{4}{c|}{WordNet: beetle - GT class: ladybug}\\
    \hline
    


     \end{tabular}\\
     
     
      \caption{$l_{1.5}$-VCEs for Madry\cite{robustness}+FT with varying radii for various ILSVRC2012 images. Each image is transformed into different classes that are part of the same WordNet synset as the original image. }
     \end{figure*}


==> panels/inverse_problem.tex <==
\begin{table}[hbt!]
       \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccc|cccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_1$:$0.99$}&\multicolumn{1}{C{.12\textwidth}}{$l_1$:$0.999$}&\multicolumn{1}{C{.12\textwidth}}{$l_1$:$0.9999$}&\multicolumn{1}{C{.12\textwidth}|}{$l_1$:$0.99999$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.99$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.999$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.9999$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.99999$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{3.6mm}
     \caption*{plane/deer}
     \includegraphics[width=1\textwidth]{inverse/init_92_from_4_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$32.1$, $l_2$:$2.6$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$39.5$, $l_2$:$3.7$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$58.1$, $l_2$:$4.2$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.9999__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$205.7$, $l_2$:$6.0$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.99999__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$63.2$, $l_2$:$1.9$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$80.2$, $l_2$:$2.4$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$106.9$, $l_2$:$3.2$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.9999__92_from_4_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$149.4$, $l_2$:$4.3$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.99999__92_from_4_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$27.4$, $l_2$:$2.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$39.9$, $l_2$:$3.0$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$54.6$, $l_2$:$3.2$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.9999__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$100.4$, $l_2$:$4.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.99999__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$60.2$, $l_2$:$1.6$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$71.0$, $l_2$:$1.9$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$80.7$, $l_2$:$2.3$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.9999__92_from_4_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$98.8$, $l_2$:$2.8$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.99999__92_from_4_wrong.png}
                
                \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{3.6mm}
     \caption*{car/truck}
     \includegraphics[width=1\textwidth]{inverse/init_20_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$6.0$, \\ $l_2$:$0.5$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$10.3$, $l_2$:$0.8$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$22.3$, $l_2$:$1.1$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.9999__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$156.4$, $l_2$:$3.9$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.99999__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$12.3$, $l_2$:$0.3$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$18.1$, $l_2$:$0.5$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$30.0$, $l_2$:$0.8$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.9999__20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$156.4$, $l_2$:$3.9$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.99999__20_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$1.1$, $l_2$:$0.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$4.0$, $l_2$:$0.3$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$14.9$, $l_2$:$0.6$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.9999__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$44.4$, $l_2$:$1.3$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.99999__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$2.3$, $l_2$:$0.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$7.5$, $l_2$:$0.2$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$18.6$, $l_2$:$0.5$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.9999__20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$41.1$, $l_2$:$1.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.99999__20_from_9_wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccc|cccc}
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_1$:$0.8$}&\multicolumn{1}{C{.12\textwidth}}{$l_1$:$0.9$}&\multicolumn{1}{C{.12\textwidth}}{$l_1$:$0.99$}&\multicolumn{1}{C{.12\textwidth}|}{$l_1$:$0.999$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.8$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.9$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.99$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:$0.999$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{3.6mm}
     \caption*{dung b/tiger }
     \includegraphics[width=1\textwidth]{inverse/init_94_from_30.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$680.0$, $l_2$:$8.4$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.8__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$1008.5$, $l_2$:$11.5$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.9__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$1373.6$, $l_2$:$14.6$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$6258.6$, $l_2$:$28.9$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$1110.6$, $l_2$:$4.9$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.8__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$1338.3$, $l_2$:$6.0$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.9__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$2530.9$, $l_2$:$10.9$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__94_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$6729.7$, $l_2$:$24.8$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__94_from_30correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$424.4$, $l_2$:$6.2$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.8__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$426.6$, $l_2$:$6.5$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.9__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$426.6$, $l_2$:$6.5$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$848.2$, $l_2$:$9.7$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$0.3$, $l_2$:$0.0$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.8__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$127.2$, $l_2$:$0.6$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.9__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$665.6$, $l_2$:$3.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__94_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$1394.6$, $l_2$:$6.2$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__94_from_30wrong.png}
                
                \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{3.6mm}
     \caption*{Pomera/French}
     \includegraphics[width=1\textwidth]{inverse/init_46_from_96.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$3195.0$, $l_2$:$19.6$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.8__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$2335.1$, $l_2$:$18.4$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.9__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$2898.5$, $l_2$:$21.7$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$3775.5$, $l_2$:$25.2$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$3089.7$, $l_2$:$11.2$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.8__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$2699.2$, $l_2$:$10.7$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.9__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$3568.1$, $l_2$:$14.2$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__46_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$:$4795.3$, $l_2$:$18.8$}
                     
     \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__46_from_96correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$1485.0$, $l_2$:$10.4$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.8__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$1914.0$, $l_2$:$12.0$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.9__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$2668.0$, $l_2$:$19.3$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.99__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$6006.9$, $l_2$:$27.6$, }
                \includegraphics[width=1\textwidth]{inverse/_l_1___0.999__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$2263.8$, $l_2$:$8.0$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.8__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$2733.3$, $l_2$:$9.5$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.9__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$4082.7$, $l_2$:$14.1$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.99__46_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$:$6484.7$, $l_2$:$22.2$, }
                \includegraphics[width=1\textwidth]{inverse/_l_2___0.999__46_from_96wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     \caption{\label{tab:inverse-vces}PM with varying threshold for $l_1, l_2$ norms.}
     \end{table}
            

==> panels/motivating_example.tex <==
\begin{table}[hbt!]
     \begin{adjustbox}{width=1\columnwidth,right}
     \centering
     \begin{tabular}{ccc}
                   \hline
                   \multicolumn{1}{c}{Orig.}&\multicolumn{1}{C{.2\textwidth}}{AFW,$l_{1.5}:50$}&\multicolumn{1}{C{.2\textwidth}}{APGD,$l_2$:12}\\
                   \hline
     \begin{subfigure}{0.2\textwidth}\centering
     
     \caption*{$\rightarrow$pirate ship, $p_i$:$0.29$}
     \includegraphics[width=1\textwidth]{afw_extended/init_afw_75_100_1.5_Madry_l2_ep364_from_72.png}
     \end{subfigure}&\begin{subfigure}{0.2\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1108.8$/$12.0$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{images/afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.2\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2615.0$/$12.0$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure} \\[1.2cm] &\begin{subfigure}{0.2\textwidth}\centering
         \includegraphics[width=1\textwidth]{images/motivating_example/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.2\textwidth}\centering
         \includegraphics[width=1\textwidth]{images/motivating_example/_l_2__12_apgd_75_l2_12_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}\\
     \hline
     \end{tabular}
     \end{adjustbox}
     \caption{\label{tab:motivating_example}$l_{1.5}$ VCEs have the right level of sparsity as can be seen from images, difference plots, and the achieved $l_1$ norm.}
     \end{table}

==> panels/pgd_fw_varying_radius.tex <==

\begin{table*}[hbt!]
     \captionsetup{font=scriptsize} 
     \begin{adjustbox}{width=2\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_2:1.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:1.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:2.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:2.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:10.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:15.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:20.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:25.0$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:cat,\\ \textbf{s}:bird}
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/init_eps_1.583_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$35.6$/$1.0$, $p_i$:$0.34$, $p_e$:$0.78$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.083_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$52.9$/$1.5$, $p_i$:$0.34$, $p_e$:$0.94$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.583_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$71.6$/$2.0$, $p_i$:$0.34$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.083_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$82.5$/$2.5$, $p_i$:$0.34$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.583_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$10.0$/$1.4$, $p_i$:$0.34$, $p_e$:$0.67$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.083_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$15.0$/$1.9$, $p_i$:$0.34$, $p_e$:$0.82$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.083_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.4$, $p_i$:$0.34$, $p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.083_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$25.0$/$2.5$, $p_i$:$0.34$, $p_e$:$0.94$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.083_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.083_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.583_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.083_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.583_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.083_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.083_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.083_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.083_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$36.7$/$1.0$, $p_i$:$0.07$, $p_e$:$0.69$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.083_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$55.9$/$1.5$, $p_i$:$0.07$, $p_e$:$0.96$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.583_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$74.9$/$2.0$, $p_i$:$0.07$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.083_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$92.2$/$2.5$, $p_i$:$0.07$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.583_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$10.0$/$1.6$, $p_i$:$0.07$, $p_e$:$0.44$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.083_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$15.0$/$1.9$, $p_i$:$0.07$, $p_e$:$0.71$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.083_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.3$, $p_i$:$0.07$, $p_e$:$0.87$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.083_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$25.0$/$2.4$, $p_i$:$0.07$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.083_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.083_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.583_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.083_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.583_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.083_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.083_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.083_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.083_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:car,\\ \textbf{s}:truck}
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/init_eps_1.520_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$36.4$/$1.0$, $p_i$:$0.17$, $p_e$:$0.95$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.020_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$55.6$/$1.5$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.520_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$74.8$/$2.0$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.020_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$94.5$/$2.5$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.520_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$10.0$/$1.1$, $p_i$:$0.17$, $p_e$:$0.78$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.020_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$15.0$/$1.5$, $p_i$:$0.17$, $p_e$:$0.92$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.020_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$1.8$, $p_i$:$0.17$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.020_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$25.0$/$2.1$, $p_i$:$0.17$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.020_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.020_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.520_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.020_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.520_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.020_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.020_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.020_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.020_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$31.3$/$1.0$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.020_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$49.5$/$1.5$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.520_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$69.7$/$2.0$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.020_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.8$/$2.5$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.520_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$10.0$/$1.4$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.020_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$15.0$/$1.9$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.020_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.020_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$25.0$/$2.3$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.020_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.020_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.520_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.020_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.520_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.020_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.020_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.020_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.020_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:plane,\\ \textbf{s}:deer}
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/init_eps_1.592_from_8_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$31.8$/$1.0$, $p_i$:$0.16$, $p_e$:$0.76$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$48.2$/$1.5$, $p_i$:$0.16$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.592_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$66.0$/$2.0$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.4$/$2.5$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.592_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$10.0$/$1.7$, $p_i$:$0.16$, $p_e$:$0.64$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$15.0$/$2.3$, $p_i$:$0.16$, $p_e$:$0.91$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.9$, $p_i$:$0.16$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$25.0$/$3.4$, $p_i$:$0.16$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.092_from_8_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.092_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.592_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.092_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.592_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.092_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.092_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.092_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.092_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$32.8$/$1.0$, $p_i$:$0.55$, $p_e$:$0.92$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$48.0$/$1.5$, $p_i$:$0.55$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.592_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$65.4$/$2.0$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$87.1$/$2.5$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.592_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$10.0$/$1.3$, $p_i$:$0.55$, $p_e$:$0.87$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$15.0$/$1.7$, $p_i$:$0.55$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_i$:$0.55$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$25.0$/$2.6$, $p_i$:$0.55$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.092_from_8_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.0__eps_1.092_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_1.5__eps_1.592_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.0__eps_2.092_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_2_2.5__eps_2.592_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_10.0__eps_10.092_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_15.0__eps_15.092_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_20.0__eps_20.092_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{apgd_varying_eps_CIFAR10/_l_1_25.0__eps_25.092_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     \caption{\label{tab:Inverse_poblem}Counterfactuals of different models using PGD for a fixed radius of the $l^2$ ball $\epsilon=2.5$.}
     \end{table*}
            
     
     
     \begin{table*}[hbt!]

 
     \begin{adjustbox}{width=2\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_{l1}:20$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:5$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:6$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:7.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:10$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:12.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:2.5}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:2.5}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:cat,\\ \textbf{s}:bird}
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/init_intersection_1.5_10_GU_impr83_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.4$, $p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$39.0$/$2.0$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$48.1$/$2.4$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$62.6$/$2.9$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$90.7$/$3.6$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$116.1$/$4.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$87.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$82.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.3$, $p_e$:$0.87$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$43.5$/$1.9$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$53.6$/$2.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$69.0$/$2.7$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.0$/$3.6$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$116.4$/$4.3$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$92.5$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$92.2$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr83_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:car,\\ \textbf{s}:truck}
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/init_intersection_1.5_10_GU_impr20_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$1.8$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$45.3$/$1.8$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$55.7$/$2.2$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$72.1$/$2.6$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$100.1$/$3.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$127.4$/$4.1$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$94.8$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$94.5$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$41.9$/$1.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$52.3$/$2.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$68.2$/$2.7$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$96.6$/$3.4$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$129.0$/$4.1$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.8$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.8$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr20_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:plane,\\ \textbf{s}:deer}
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/init_intersection_1.5_10_GU_impr92_from_8_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.9$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$38.0$/$2.0$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$47.2$/$2.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$59.9$/$2.9$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$82.9$/$3.7$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$111.0$/$4.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.7$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.4$/$2.5$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$38.1$/$2.0$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$47.7$/$2.4$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$62.3$/$2.8$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$92.7$/$3.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$122.6$/$4.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$86.7$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$87.1$/$2.5$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_l1_20__apgd_75_l1_20_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_5__intersection_1.5_5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_6__intersection_1.5_6_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_7.5__intersection_1.5_7.5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_10__intersection_1.5_10_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_1.5_12.5__intersection_1.5_12.5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_intersection_l2_2.5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_varying_eps_CIFAR10/_l_2__2.5_apgd_75_l2_2.5_GU_impr92_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     \caption{\label{tab:Inverse_poblem}VCEs of RATIO for CIFAR10 and of Madryl2-ep1 for IMAGENET1000 generated with A-PGD in the $l_2$ and $l_1$ ball with varying radius.}
     \end{table*}
     
     \begin{table*}[hbt!]
     \begin{adjustbox}{width=2\columnwidth,center}
     \centering
     \begin{tabular}{cccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_{l1}:400$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:50$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:70$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:90$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:100$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:120$}&\multicolumn{1}{C{.12\textwidth}}{$l_{1.5}:140$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:12}&\multicolumn{1}{C{.12\textwidth}}{$l_2$:12}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:cauliflower,\\ \textbf{s}:head cabbage}
     \includegraphics[width=1\textwidth]{afw_extended/init_afw_75_100_1.5_Madry_l2_ep337_from_93.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$10.3$, $p_e$:$0.75$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1476.0$/$10.1$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2115.8$/$13.7$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2686.8$/$16.6$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3035.7$/$18.2$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3745.8$/$21.1$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$4481.0$/$24.0$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2978.4$/$11.9$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3020.3$/$12.0$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$11.2$, $p_e$:$0.85$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1710.2$/$9.5$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2465.1$/$12.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3198.9$/$16.3$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3527.4$/$17.8$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$4216.2$/$20.7$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$5038.8$/$23.8$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3477.8$/$11.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3491.7$/$12.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep337_from_93wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:pirate, pira,\\ \textbf{s}:catamaran}
     \includegraphics[width=1\textwidth]{afw_extended/init_afw_75_100_1.5_Madry_l2_ep364_from_72.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$14.5$, $p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1108.8$/$12.0$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1701.0$/$15.7$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2312.4$/$19.1$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2629.9$/$20.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3238.0$/$23.2$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3911.7$/$25.7$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2541.2$/$11.9$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2615.0$/$12.0$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep364_from_72correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep364_from_72correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$12.0$, $p_e$:$0.62$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1398.3$/$10.7$, $p_e$:$0.82$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1804.6$/$15.0$, $p_e$:$0.96$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2547.4$/$18.0$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2873.3$/$19.8$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3636.0$/$22.4$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$4276.7$/$25.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2934.5$/$11.9$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2926.7$/$12.0$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep364_from_72wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep364_from_72wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:reflex camer,\\ \textbf{s}:red wine}
     \includegraphics[width=1\textwidth]{afw_extended/init_afw_75_100_1.5_Madry_l2_ep372_from_96.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$13.9$, $p_e$:$0.39$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1335.8$/$11.0$, $p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1976.2$/$14.6$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2682.8$/$17.9$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3031.7$/$19.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3755.3$/$22.7$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$4401.9$/$25.8$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2877.7$/$11.9$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2889.7$/$12.0$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$14.9$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1541.0$/$10.3$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2261.7$/$13.6$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2905.1$/$16.7$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3310.4$/$18.1$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3919.5$/$21.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$4679.8$/$23.4$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3207.1$/$11.8$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3228.4$/$12.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep372_from_96wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:dung beetle,\\ \textbf{s}:tiger beetle}
     \includegraphics[width=1\textwidth]{afw_extended/init_afw_75_100_1.5_Madry_l2_ep394_from_30.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$400.0$/$11.4$, $p_e$:$0.87$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1381.0$/$10.6$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1995.8$/$13.7$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2492.2$/$16.6$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2852.1$/$18.3$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$3583.8$/$20.4$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$4125.8$/$22.2$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2817.6$/$11.8$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2845.6$/$12.0$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$400.0$/$11.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1263.1$/$11.2$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1875.2$/$14.8$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2584.6$/$17.7$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2872.1$/$18.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3364.7$/$20.4$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$3649.5$/$21.7$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2706.8$/$11.9$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2793.7$/$12.0$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_l1_400__apgd_75_l1_400_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_50__afw_75_50_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_70__afw_75_70_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_90__afw_75_90_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_100__afw_75_100_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_120__afw_75_120_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_1.5_140__afw_75_140_1.5_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_afw_75_12_l2_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{afw_extended/_l_2__12_apgd_75_l2_12_Madry_l2_ep394_from_30wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     \caption{\label{tab:Inverse_poblem}Counterfactuals of different models using PGD for a fixed radius of the $l^2$ ball $\epsilon=2.5$.}
     \end{table*}
            
            
            
            

==> panels/pgd_varying_radius.tex <==
\begin{table}[hbt!]
    \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_2:1.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:1.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:2.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:2.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:10.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:15.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:20.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:25.0$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:plane,\\ \textbf{s}:deer}
     \includegraphics[width=1\textwidth]{apgd/init_eps_1.592_from_8_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$31.8$/$1.0$, $p_i$:$0.16$, $p_e$:$0.76$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_1.0__eps_1.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$48.2$/$1.5$, $p_i$:$0.16$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_1.5__eps_1.592_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$66.0$/$2.0$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_2.0__eps_2.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.4$/$2.5$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_2.5__eps_2.592_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$10.0$/$1.7$, $p_i$:$0.16$, $p_e$:$0.64$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_10.0__eps_10.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$15.0$/$2.3$, $p_i$:$0.16$, $p_e$:$0.91$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_15.0__eps_15.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.9$, $p_i$:$0.16$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_20.0__eps_20.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$25.0$/$3.4$, $p_i$:$0.16$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_25.0__eps_25.092_from_8_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$32.8$/$1.0$, $p_i$:$0.55$, $p_e$:$0.92$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_1.0__eps_1.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$48.0$/$1.5$, $p_i$:$0.55$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_1.5__eps_1.592_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$65.4$/$2.0$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_2.0__eps_2.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$87.1$/$2.5$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_2.5__eps_2.592_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$10.0$/$1.3$, $p_i$:$0.55$, $p_e$:$0.87$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_10.0__eps_10.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$15.0$/$1.7$, $p_i$:$0.55$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_15.0__eps_15.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_i$:$0.55$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_20.0__eps_20.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$25.0$/$2.6$, $p_i$:$0.55$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_25.0__eps_25.092_from_8_wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_2:6.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:8.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:10.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:12.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:600.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:800.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:1000.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:1200.0$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:dung beetle,\\ \textbf{s}:tiger beetle}
     \includegraphics[width=1\textwidth]{apgd_IN1k/init_eps_1000.094_from_30.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1322.7$/$6.0$, $p_i$:$0.04$, $p_e$:$0.91$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_6.0__eps_6.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1777.4$/$8.0$, $p_i$:$0.04$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_8.0__eps_8.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2307.2$/$10.0$, $p_i$:$0.04$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_10.0__eps_10.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2845.6$/$12.0$, $p_i$:$0.04$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_12.0__eps_12.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$600.0$/$14.1$, $p_i$:$0.04$, $p_e$:$0.96$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_600.0__eps_600.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$800.0$/$16.1$, $p_i$:$0.04$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_800.0__eps_800.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1000.0$/$17.8$, $p_i$:$0.04$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1000.0__eps_1000.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1200.0$/$18.3$, $p_i$:$0.04$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1200.0__eps_1200.094_from_30correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1322.0$/$6.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_6.0__eps_6.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1783.5$/$8.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_8.0__eps_8.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2241.7$/$10.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_10.0__eps_10.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2793.7$/$12.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_12.0__eps_12.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$600.0$/$14.8$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_600.0__eps_600.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$800.0$/$17.2$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_800.0__eps_800.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1000.0$/$19.4$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1000.0__eps_1000.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1200.0$/$22.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1200.0__eps_1200.094_from_30wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     \caption{\label{tab:Inverse_poblem}VCEs of RATIO for CIFAR10 and of Madryl2-ep1 for IMAGENET1000 generated with A-PGD in the $l_2$ and $l_1$ ball with varying radius.}
     \end{table}
            

==> panels/pgd_varying_radius_one_fixed.tex <==
\begin{table}[hbt!]
    \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_2:1.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:1.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:2.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:2.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:10.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:15.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:20.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:25.0$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:plane,\\ \textbf{s}:deer}
     \includegraphics[width=1\textwidth]{apgd/init_eps_1.592_from_8_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$31.8$/$1.0$, $p_i$:$0.15$, $p_e$:$0.76$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_1.0__eps_1.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$48.2$/$1.5$, $p_i$:$0.15$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_1.5__eps_1.592_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$66.0$/$2.0$, $p_i$:$0.15$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_2.0__eps_2.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.4$/$2.5$, $p_i$:$0.15$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_2_2.5__eps_2.592_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$10.0$/$1.7$, $p_i$:$0.15$, $p_e$:$0.64$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_10.0__eps_10.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$15.0$/$2.3$, $p_i$:$0.15$, $p_e$:$0.91$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_15.0__eps_15.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$20.0$/$2.9$, $p_i$:$0.15$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_20.0__eps_20.092_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$25.0$/$3.4$, $p_i$:$0.15$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd/_l_1_25.0__eps_25.092_from_8_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$32.8$/$1.0$, $p_i$:$0.15$, $p_e$:$0.92$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_1.0__eps_1.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$48.0$/$1.5$, $p_i$:$0.15$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_1.5__eps_1.592_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$65.4$/$2.0$, $p_i$:$0.15$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_2.0__eps_2.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$87.1$/$2.5$, $p_i$:$0.15$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd/_l_2_2.5__eps_2.592_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$10.0$/$1.3$, $p_i$:$0.15$, $p_e$:$0.87$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_10.0__eps_10.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$15.0$/$1.7$, $p_i$:$0.15$, $p_e$:$0.94$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_15.0__eps_15.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$20.0$/$2.2$, $p_i$:$0.15$, $p_e$:$0.98$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_20.0__eps_20.092_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$25.0$/$2.6$, $p_i$:$0.15$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{apgd/_l_1_25.0__eps_25.092_from_8_wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{$l_2:6.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:8.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:10.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_2:12.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:600.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:800.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:1000.0$}&\multicolumn{1}{C{.12\textwidth}}{$l_1:1200.0$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:dung beetle,\\ \textbf{s}:tiger beetle}
     \includegraphics[width=1\textwidth]{apgd_IN1k/init_eps_1000.094_from_30.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1322.7$/$6.0$, $p_i$:$0.04$, $p_e$:$0.91$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_6.0__eps_6.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1777.4$/$8.0$, $p_i$:$0.04$, $p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_8.0__eps_8.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2307.2$/$10.0$, $p_i$:$0.04$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_10.0__eps_10.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$2845.6$/$12.0$, $p_i$:$0.04$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_12.0__eps_12.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$600.0$/$14.1$, $p_i$:$0.04$, $p_e$:$0.96$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_600.0__eps_600.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$800.0$/$16.1$, $p_i$:$0.04$, $p_e$:$0.98$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_800.0__eps_800.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1000.0$/$17.8$, $p_i$:$0.04$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1000.0__eps_1000.094_from_30correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$1200.0$/$18.3$, $p_i$:$0.04$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1200.0__eps_1200.094_from_30correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1322.0$/$6.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_6.0__eps_6.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1783.5$/$8.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_8.0__eps_8.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2241.7$/$10.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_10.0__eps_10.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$2793.7$/$12.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_2_12.0__eps_12.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$600.0$/$14.8$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_600.0__eps_600.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$800.0$/$17.2$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_800.0__eps_800.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1000.0$/$19.4$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1000.0__eps_1000.094_from_30wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$1200.0$/$22.0$, $p_i$:$0.85$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{apgd_IN1k/_l_1_1200.0__eps_1200.094_from_30wrong.png}
                
                \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     \caption{\label{tab:Inverse_poblem}VCEs of RATIO for CIFAR10 and of Madryl2-ep1 for IMAGENET1000 generated with A-PGD in the $l_2$ and $l_1$ ball with varying radius.}
     \end{table}
            

==> panels/prior_benchmark_fig.tex <==
\begin{figure*}[t]
     
     \centering
     \begin{tabular}{cccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{BiT-M\cite{KolesnikovEtAl2019}}&\multicolumn{1}{C{.12\textwidth}}{RST-s\cite{CarEtAl19}}&\multicolumn{1}{C{.12\textwidth}}{RATIO\cite{augustin2020}}&\multicolumn{1}{C{.12\textwidth}}{GU\cite{gowal2020uncovering}}&\multicolumn{1}{C{.12\textwidth}}{GU+FT\cite{croce2021adversarial}}&\multicolumn{1}{C{.12\textwidth}}{PAT\cite{laidlaw2020perceptual}}&\multicolumn{1}{C{.12\textwidth}}{HenC\cite{hendrycks2020augmix}}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
      \caption*{$\rightarrow$car,\\ $\rightarrow$truck}
     \includegraphics[width=1\textwidth]{prior/init_Gowal2020Uncovering_improved20_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.98$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust20_from_1_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.47$, \\$p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab20_from_1_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.22$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L220_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.54$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L220_from_1_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.17$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.43$, \\$p_e$:$0.74$}
                     
     \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved20_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.96$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions20_from_1_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust20_from_1_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab20_from_1_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L220_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L220_from_1_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved20_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions20_from_1_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.01$, \\$p_e$:$0.99$}
                    \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust20_from_1_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.51$, \\$p_e$:$0.99$}
                    \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab20_from_1_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.78$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L220_from_9_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.44$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L220_from_1_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.83$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved20_from_9_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.57$, \\$p_e$:$0.87$}
                    \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved20_from_9_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.04$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions20_from_1_wrong.png}
                    
                    \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust20_from_1_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab20_from_1_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L220_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L220_from_1_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved20_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved20_from_9_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions20_from_1_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}\\ 
     \hline
     
     \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$\rightarrow$frog,\\ $\rightarrow$plane}
     \includegraphics[width=1\textwidth]{prior/init_Gowal2020Uncovering_improved19_from_6_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.99$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust19_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.20$, \\$p_e$:$0.82$}
                     
     \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab19_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.41$, \\$p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L219_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.57$, \\$p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L219_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.32$, \\$p_e$:$0.97$}
                     
     \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved19_from_6_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.25$, \\$p_e$:$0.90$}
                     
     \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved19_from_0_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$p_i$:$0.99$, \\$p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions19_from_6_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust19_from_6_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab19_from_6_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L219_from_6_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L219_from_6_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved19_from_6_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved19_from_0_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions19_from_6_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.00$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust19_from_6_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.17$, \\$p_e$:$0.95$}
                    \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab19_from_6_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.11$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L219_from_6_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.08$, \\$p_e$:$0.99$}
                    \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L219_from_6_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.19$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved19_from_6_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.50$, \\$p_e$:$0.97$}
                    \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved19_from_0_wrong.png}
                    
                    \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                    
                    \caption*{$p_i$:$0.00$, \\$p_e$:$1.00$}
                    \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions19_from_6_wrong.png}
                    
                    \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/BiT-M-R,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__BiT-M-R50x1_CIFAR10_nonrobust19_from_6_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/rst_sta,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__rst_stab19_from_6_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Augusti,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Augustin2020Adversarial_34_10_extra-L219_from_6_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_extra-L219_from_6_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Gowal20,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Gowal2020Uncovering_improved19_from_6_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/PAT_imp,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__PAT_improved19_from_0_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                         \includegraphics[width=1\textwidth]{prior/Hendryc,!l_2_-pVCE,_epsilon=2.5___2.5_2_2.5__Hendrycks2020AugMix_ResNeXt-corruptions19_from_6_wrong_diff_abs_scaled.png}
                         
                         \end{subfigure}\\ 
     \hline
     \end{tabular}
     
     \caption{\textbf{CIFAR10:} \label{tab:prior_benchmark}$l_2$-pVCEs of different classifiers used in \cref{tab:benchmark-cifar10} for $\epsilon_2=2.5$. The difference plots are much less sparse due to the noise used during the generation of $l_2$-pVCEs. Note, that even using generative prior doesn't help to generate VCEs which introduce class-specific features for non-robust models, such as \textit{BiT-M} and \textit{HenC}. Please see target class ``truck'' in the first example for the counterfactual of a ``car'' image and in the lower panel target class ``plane'' for an original image of a frog. In both cases the $l_2$-pVCEs for \textit{BiT-M} and \textit{HenC} show almost no changes of the original image.}
     \end{figure*}
            

==> panels/prior_vs_pgd.tex <==
\begin{table}[hbt!]
      \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{ccccccccc}
                   \hline
                   \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.12\textwidth}}{APGD,$l_2$:$2.5$}&\multicolumn{1}{C{.12\textwidth}}{PSGLA,$l_2$:$2.5$}&\multicolumn{1}{C{.12\textwidth}}{APGD,$l_2$:$5$}&\multicolumn{1}{C{.12\textwidth}}{PSGLA,$l_2$:$5$}&\multicolumn{1}{C{.12\textwidth}}{APGD,$l_1$:$50$}&\multicolumn{1}{C{.12\textwidth}}{PSGLA,$l_1$:$50$}&\multicolumn{1}{C{.12\textwidth}}{APGD,$l_1$:$100$}&\multicolumn{1}{C{.12\textwidth}}{PSGLA,$l_1$:$100$}\\
                   \hline
                   \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:plane,\\ \textbf{s}:deer}
     \includegraphics[width=1\textwidth]{pgd&prior/init_apgd_75_100_l192_from_8_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$84.4$/$2.5$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l292_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$99.0$/$2.5$, $p_i$:$0.16$, $p_e$:$0.99$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l292_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$206.5$/$5.0$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l292_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$187.4$/$5.0$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l292_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$50.0$/$5.0$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l192_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$46.8$/$1.3$, $p_i$:$0.16$, $p_e$:$0.67$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l192_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$100.0$/$7.2$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l192_from_8_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$95.3$/$2.9$, $p_i$:$0.16$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l192_from_8_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l292_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l292_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l292_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l292_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l192_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l192_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l192_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l192_from_8_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$87.1$/$2.5$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l292_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$93.5$/$2.5$, $p_i$:$0.55$, $p_e$:$0.99$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l292_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$204.2$/$5.0$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l292_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$196.8$/$5.0$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l292_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$50.0$/$3.7$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l192_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$46.4$/$1.2$, $p_i$:$0.55$, $p_e$:$0.86$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l192_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$100.0$/$5.2$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l192_from_8_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$97.2$/$2.8$, $p_i$:$0.55$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l192_from_8_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l292_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l292_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l292_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l292_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l192_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l192_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l192_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l192_from_8_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{\textbf{t}:car,\\ \textbf{s}:truck}
     \includegraphics[width=1\textwidth]{pgd&prior/init_apgd_75_100_l120_from_9_.png}
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$94.5$/$2.5$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l220_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$104.7$/$2.5$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l220_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$202.3$/$5.0$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l220_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$207.0$/$5.0$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l220_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$50.0$/$3.5$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l120_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$49.6$/$1.2$, $p_i$:$0.17$, $p_e$:$0.84$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l120_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$100.0$/$5.0$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l120_from_9_correct.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{$l_1$/$l_2$:$99.3$/$2.5$, $p_i$:$0.17$, $p_e$:$1.00$}
                     
     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l120_from_9_correct.png}
     
     \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l220_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l220_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l220_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l220_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l120_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l120_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l120_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
         \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l120_from_9_correct_diff_abs_scaled.png}
         
         \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$91.8$/$2.5$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$101.1$/$2.5$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$206.6$/$5.0$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$208.4$/$5.0$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$50.0$/$3.5$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l120_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$48.5$/$1.3$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l120_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$100.0$/$5.0$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l120_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{$l_1$/$l_2$:$98.0$/$2.5$, $p_i$:$0.83$, $p_e$:$1.00$}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l120_from_9_wrong.png}
                
                \end{subfigure}\\&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l220_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l220_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l220_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l220_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___50__apgd_75_50_l120_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___50__nsigma_50_l120_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_1___100__apgd_75_100_l120_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                     \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_1___100__nsigma_100_l120_from_9_wrong_diff_abs_scaled.png}
                     
                     \end{subfigure}\\ 
     \hline
     \end{tabular}
     \end{adjustbox}
     
     
      \begin{adjustbox}{width=0.6\columnwidth,center}
   \centering
  \begin{tabular}{c|c|c}
    \backslashbox{Model}{FID(ID/OD)$\downarrow$} & PSGLA,$l_2$:$2.5$ & APGD,$l_2$:$2.5$ \\
    \hline
    GU-extra & 9.1/48 & 14.8/54.2 \\
    GU-extra\_ep1 & 7.6/46.2 &  \cellcolor{green!25} 10/41.2 \\
    \hline
  \end{tabular}
  \end{adjustbox}
  
     \caption{\label{tab:Inverse_poblem}PSGLA vs. APGD constrained to $l^1, l^2$ balls of varying radius.}
     \end{table}
            

==> panels/prior_vs_pgd_short.tex <==
\begin{figure}[t]
       
     \centering
     \begin{tabular}{ccccc}
                   \hline
                
                   \multicolumn{1}{c}{Original} &\multicolumn{1}{C{.12\textwidth}}{\footnotesize $l_2$-VCE, $\epsilon=2.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$-pVCE, $\epsilon=2.5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$-VCE,$\;$ $\epsilon=5$}&\multicolumn{1}{C{.12\textwidth}}{$l_2$-pVCE, $\epsilon=5$}\\
                   \hline
                 
        \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{{\footnotesize truck:0.83\\
     $\rightarrow$truck}}
     \includegraphics[width=1\textwidth]{pgd&prior/init_nsigma_2.5_l220_from_9_.png}
     \end{subfigure}
    &\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize $l_1$/$l_2$:$91.8$/$2.5$,
                truck:$1.00$}}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___2.5__apgd_75_2.5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize$l_1$/$l_2$:$101.1$/$2.5$, truck:$1.00$}}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___2.5__nsigma_2.5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{ \footnotesize$l_1$/$l_2$:$206.6$/$5.0$, truck:$1.00$}}
                \includegraphics[width=1\textwidth]{pgd&prior/APGD,_l_2___5__apgd_75_5_l220_from_9_wrong.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize$l_1$/$l_2$:$208.4$/$5.0$, truck:$1.00$}}
                \includegraphics[width=1\textwidth]{pgd&prior/PSGLA,_l_2___5__nsigma_5_l220_from_9_wrong.png}
                
                \end{subfigure}\\
                \begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{{\footnotesize cat:0.35\\
     $\rightarrow$cat}}
     \includegraphics[width=1\textwidth]{images/benchmark_folder_CIFAR10/init.png}
     \end{subfigure}
    &\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize$l_1$/$l_2$:$94.5$/$2.5$,
                cat:$1.00$}}
                \includegraphics[width=1\textwidth]{images/benchmark_folder_CIFAR10/GU_impr.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize$l_1$/$l_2$:$104.5$/$2.5$, cat:$0.98$}}
                \includegraphics[width=1\textwidth]{pgd&prior/ood_prior_vs_apgd_vce_prior_2_5.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize$l_1$/$l_2$:$216.0$/$5.0$, cat:$1.00$}}
                \includegraphics[width=1\textwidth]{images/pgd&prior/ood_prior_vs_apgd_vce_apgd_5.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{{\footnotesize$l_1$/$l_2$:$213.2$/$5.0$, cat:$1.00$}}
                \includegraphics[width=1\textwidth]{images/pgd&prior/ood_prior_vs_apgd_vce_prior_5.png}
                
                \end{subfigure}\\
                
     \end{tabular}
    
     \caption{\label{fig:prior_vs_apgd}PALMC vs. APGD used to generate $l_2$-(p)VCEs 
     for $\epsilon \in \{2.5, 5\}$. In order to see stronger changes for pVCEs, one needs to increase the radius, which generates good images, but lacks the subtle changes we see for VCEs for smaller budget.}
     \end{figure}
            
            


==> panels/rebuttal/apgd_prior.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure}[hbt!]
\vspace{-4mm}
     \centering
     \small
     \vspace{-1mm}
     \centering
     \small
     \begin{tabular}{c|cc|cc}
     \hline
     {{\footnotesize Original}
     } & 
     {{\footnotesize $l_{\infty}$, $\epsilon = 0.03$}
     } & 
      {{\footnotesize diff.}
     } & 

     {{\footnotesize $l_{1.5}$, $\epsilon = 50$}
     } &
     {{\footnotesize diff.}
     }\\
     \hline
     \begin{subfigure}{0.09\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/linf/94_from_300_to_300_start=0.85378,end=0.99973_l_0_150255.0,l_1_4180.19,l_2_11.03,l_inf_0.03first.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/linf/94_from_300_to_305_start=0.03822,end=0.79210_l_0_150333.0,l_1_2921.90,l_2_7.60,l_inf_0.02last.png}
     \end{subfigure} &
     
     \begin{subfigure}{0.09\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/diff_plots/rebuttal_linf_diff.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/ablation_imagenet_1_5/l2_ep3_Madry_l2_improved_ep_394_from_30correct.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/diff_plots/rebuttal_1_5_diff.png}
     \end{subfigure}
     \end{tabular}
    
    
     {\small \begin{flushleft}Figure B. $l_\infty$- and $l_{1.5}$-VCEs into correct class "dung beetle".\end{flushleft}}
     \vspace{-1mm}
     
     
     \begin{tabular}{c|c|cc|cc}
     \hline
     {{\footnotesize \scriptsize{Waterm. Train.}}
     } & 
     {{\footnotesize Original}
     } &
     {{\footnotesize $l_{2}$-VCE}
     } & 
      {{\footnotesize diff.}
     } & 
     {{\footnotesize pVCE}
     } &
     {{\footnotesize diff.}
     }\\
     \hline
     \begin{subfigure}{0.075\textwidth}\centering
     
      
       \includegraphics[width=1\textwidth]{images/rebuttal/apgd_prior/bird_watermark_trainset.png}
     
    
    
     \end{subfigure} &
     \begin{subfigure}{0.075\textwidth}\centering
     
     
     \includegraphics[width=1\textwidth]{images/rebuttal/apgd_prior/328_from_0_to_2_start=0.00029,end=1.00000_l_0_3072.0,l_1_184.93,l_2_4.99,l_inf_0.44first.png}
    
    
     \end{subfigure} &
     \begin{subfigure}{0.075\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/apgd_prior/328_from_0_to_2_start=0.00029,end=1.00000_l_0_3072.0,l_1_184.93,l_2_4.99,l_inf_0.44last.png}
    
    
     \end{subfigure} &
     \begin{subfigure}{0.075\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/diff_plots/rebuttal_apgd_diff_3.png}
    
    
     \end{subfigure} &
     \begin{subfigure}{0.075\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/apgd_prior/328_from_0_to_2_start=0.00029,end=0.99863_l_0_3072.0,l_1_178.83,l_2_5.00,l_inf_0.48last.png}
    
    
     \end{subfigure} &
     \begin{subfigure}{0.075\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/diff_plots/rebuttal_prior_diff_3.png}
     
     
     \end{subfigure}
     \end{tabular}
    
    
     {\small \begin{flushleft}Figure C. pVCE hide the watermark artefacts shown by $l_{2}$-VCE.\end{flushleft}}
     \vspace{-4mm}
     \end{figure}


==> panels/rebuttal/imagenet_s_segmentation.tex <==
\setlength{\tabcolsep}{1pt}




\setlength{\tabcolsep}{1pt}
\begin{figure}[hbt!]
\vspace{-2mm}
     \centering
     \small
     \begin{tabular}{c|cc|cc}
     \hline
     {{goldfinch}
     } & 
     {{\footnotesize $l_{1.5}$, $\epsilon=50$}
     } &
    {{\footnotesize $\epsilon=75$}
     } &
     {{\footnotesize $l_{2}$, $\epsilon=12$}
     } &
     {{\footnotesize $\epsilon=18$}
     }
     \\
     \hline
     \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/gt.png}
     \end{subfigure} &
      \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l15_1.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l15_2.png}
     \end{subfigure} &
      \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l2_1.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l2_2.png}
     \end{subfigure}\\
     \hline
     Mask & {\footnotesize $\mathbb{E}[d] = 1.3$}  & {\footnotesize $\mathbb{E}[d] = 3.1$}  & {\footnotesize $\mathbb{E}[d] = 11.4$}  & {\footnotesize $\mathbb{E}[d] = 16.1$} \\
      \hline
     \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/masked.png}
     \end{subfigure} &
      \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l15_1_diff.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l15_2_diff.png}
     \end{subfigure} &
      \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l2_1_diff.png}
     \end{subfigure} &
     \begin{subfigure}{0.09\textwidth}\centering
     \includegraphics[width=1\textwidth]{images/rebuttal/imagenet_s/l2_2_diff.png}
     \end{subfigure}
     \end{tabular}
    
    
     
     {\small \begin{flushleft}Figure A. VCEs for "goldfinch $\rightarrow$ house finch".\end{flushleft}}
     \vspace{-4mm}
 \end{figure}

==> panels/rebuttal/linf_vces.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure}[hbt]
\vspace{-1mm}
     \centering
     \small
     \begin{tabular}{c|cc|cc}
     \hline
     {{\footnotesize Original}
     } & 
     {{\footnotesize $l_{\infty}$, $\epsilon = 0.03$}
     } & 
      {{\footnotesize diff.}
     } & 

     {{\footnotesize $l_{1.5}$, $\epsilon = 50$}
     } &
     {{\footnotesize diff.}
     }\\
     \hline
     \begin{subfigure}{0.08\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/linf/94_from_300_to_300_start=0.85378,end=0.99973_l_0_150255.0,l_1_4180.19,l_2_11.03,l_inf_0.03first.png}
     \end{subfigure} &
     \begin{subfigure}{0.08\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/linf/94_from_300_to_305_start=0.03822,end=0.79210_l_0_150333.0,l_1_2921.90,l_2_7.60,l_inf_0.02last.png}
     \end{subfigure} &
     
     \begin{subfigure}{0.08\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/diff_plots/rebuttal_linf_diff.png}
     \end{subfigure} &
     \begin{subfigure}{0.08\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/ablation_imagenet_1_5/l2_ep3_Madry_l2_improved_ep_394_from_30correct.png}
     \end{subfigure} &
     \begin{subfigure}{0.08\textwidth}\centering
     
     \includegraphics[width=1\textwidth]{images/rebuttal/diff_plots/rebuttal_1_5_diff.png}
     \end{subfigure}
     \end{tabular}
    
    
     {\small \begin{flushleft}Figure B. $l_\infty$- and $l_{1.5}$-VCEs into correct class "dung beetle".\end{flushleft}}
     \vspace{-5mm}
     \end{figure}


==> panels/table-inverse_smaller_radius_latex_images.tex <==
\begin{table*}[hbt!]
      \begin{adjustbox}{width=0.5\columnwidth,center}
     \centering
     \begin{tabular}{ccccc}
                   \hline
                   Dataset-$p$ & \multicolumn{1}{c}{Orig.} & \multicolumn{1}{C{.20\textwidth}}{0.25eps \par (FID:NA) \par (FID_{TI}:NA)}&\multicolumn{1}{C{.20\textwidth}}{0.1eps \par (FID:NA) \par (FID_{TI}:NA)}&\multicolumn{1}{C{.20\textwidth}}{0.02eps \par (FID:NA) \par (FID_{TI}:NA)}\\
                   \hline
                   \parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{CIFAR10-$\ell^2$}}}
                   & \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{26.8mm}
     \caption*{deer/horse}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/init_5_from_horse_to_deer_start=0.24675,end=0.99976_l_0_3022.0,l_1_46.24,l_2_1.28,l_inf_0.17,LPIPS_0.32_first.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{deer:$0.52$, $p:1.00$, $p_R:0.58$, $p_{NR}:0.95$, $p_{RA}:0.89$, $MSE: 0.98$, $MSE_c: 1.05$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_5_from_horse_to_deer_start=0.51990,end=0.99975_l_0_3020.0,l_1_66.14,l_2_1.79,l_inf_0.21,LPIPS_0.32_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{deer:$0.22$, $p:0.00$, $p_R:0.01$, $p_{NR}:0.09$, $p_{RA}:0.11$, $MSE: 19.75$, $MSE_c: 19.95$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_5_from_horse_to_deer_start=0.22148,end=0.00362_l_0_2972.0,l_1_1550.73,l_2_31.49,l_inf_1.00,LPIPS_0.86_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{deer:$0.25$, $p:1.00$, $p_R:0.45$, $p_{NR}:0.92$, $p_{RA}:0.54$, $MSE: 0.91$, $MSE_c: 1.04$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_5_from_horse_to_deer_start=0.24675,end=0.99976_l_0_3022.0,l_1_46.24,l_2_1.28,l_inf_0.17,LPIPS_0.32_last.png}
     
     \end{subfigure}\\ &&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{horse:$0.27$, $p:1.00$, $p_R:0.97$, $p_{NR}:0.97$, $p_{RA}:0.89$, $MSE: 0.95$, $MSE_c: 1.10$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_5_from_horse_to_horse_start=0.27317,end=0.99976_l_0_3011.0,l_1_78.03,l_2_2.12,l_inf_0.26,LPIPS_0.39_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{horse:$0.37$, $p:1.00$, $p_R:0.88$, $p_{NR}:0.96$, $p_{RA}:0.85$, $MSE: 0.96$, $MSE_c: 1.08$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_5_from_horse_to_horse_start=0.36869,end=0.99976_l_0_2969.0,l_1_53.02,l_2_1.54,l_inf_0.19,LPIPS_0.31_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{horse:$0.47$, $p:1.00$, $p_R:0.94$, $p_{NR}:0.95$, $p_{RA}:0.85$, $MSE: 0.91$, $MSE_c: 1.09$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_5_from_horse_to_horse_start=0.47031,end=0.99976_l_0_2915.0,l_1_58.43,l_2_1.56,l_inf_0.16,LPIPS_0.36_last.png}
                
                \end{subfigure}\\& \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{26.8mm}
     \caption*{cat/dog}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/init_11_from_dog_to_cat_start=0.81059,end=0.99975_l_0_3072.0,l_1_24.54,l_2_0.70,l_inf_0.09,LPIPS_0.16_first.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{cat:$0.69$, $p:1.00$, $p_R:0.97$, $p_{NR}:0.89$, $p_{RA}:0.99$, $MSE: 0.99$, $MSE_c: 2.27$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_11_from_dog_to_cat_start=0.68999,end=0.99976_l_0_3072.0,l_1_73.61,l_2_1.93,l_inf_0.18,LPIPS_0.31_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{cat:$0.62$, $p:1.00$, $p_R:0.95$, $p_{NR}:0.91$, $p_{RA}:0.88$, $MSE: 1.00$, $MSE_c: 2.21$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_11_from_dog_to_cat_start=0.62435,end=0.99975_l_0_3072.0,l_1_45.68,l_2_1.25,l_inf_0.13,LPIPS_0.24_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{cat:$0.81$, $p:1.00$, $p_R:0.85$, $p_{NR}:0.93$, $p_{RA}:0.68$, $MSE: 1.05$, $MSE_c: 2.10$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_11_from_dog_to_cat_start=0.81059,end=0.99975_l_0_3072.0,l_1_24.54,l_2_0.70,l_inf_0.09,LPIPS_0.16_last.png}
     
     \end{subfigure}\\ &&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{dog:$0.29$, $p:1.00$, $p_R:0.99$, $p_{NR}:0.89$, $p_{RA}:1.00$, $MSE: 0.96$, $MSE_c: 1.04$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_11_from_dog_to_dog_start=0.28981,end=0.99973_l_0_3072.0,l_1_47.85,l_2_1.65,l_inf_0.35,LPIPS_0.37_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{dog:$0.36$, $p:1.00$, $p_R:0.94$, $p_{NR}:0.92$, $p_{RA}:0.98$, $MSE: 0.94$, $MSE_c: 1.12$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_11_from_dog_to_dog_start=0.36454,end=0.99975_l_0_3072.0,l_1_38.31,l_2_1.19,l_inf_0.36,LPIPS_0.33_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{dog:$0.18$, $p:1.00$, $p_R:0.88$, $p_{NR}:0.93$, $p_{RA}:0.89$, $MSE: 1.01$, $MSE_c: 1.13$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_11_from_dog_to_dog_start=0.18334,end=0.99976_l_0_3072.0,l_1_29.33,l_2_0.93,l_inf_0.29,LPIPS_0.27_last.png}
                
                \end{subfigure}\\& \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{26.8mm}
     \caption*{car/truck}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/init_20_from_truck_to_car_start=0.55615,end=0.99975_l_0_3072.0,l_1_39.75,l_2_1.05,l_inf_0.11,LPIPS_0.19_first.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{car:$0.67$, $p:1.00$, $p_R:0.98$, $p_{NR}:0.94$, $p_{RA}:1.00$, $MSE: 0.61$, $MSE_c: 1.34$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_20_from_truck_to_car_start=0.66756,end=0.99976_l_0_3072.0,l_1_46.77,l_2_1.19,l_inf_0.13,LPIPS_0.21_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{car:$0.54$, $p:1.00$, $p_R:0.98$, $p_{NR}:0.93$, $p_{RA}:1.00$, $MSE: 0.60$, $MSE_c: 1.34$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_20_from_truck_to_car_start=0.53686,end=0.99976_l_0_3072.0,l_1_52.05,l_2_1.33,l_inf_0.15,LPIPS_0.23_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{car:$0.56$, $p:1.00$, $p_R:0.96$, $p_{NR}:0.93$, $p_{RA}:1.00$, $MSE: 0.59$, $MSE_c: 1.28$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_20_from_truck_to_car_start=0.55615,end=0.99975_l_0_3072.0,l_1_39.75,l_2_1.05,l_inf_0.11,LPIPS_0.19_last.png}
     
     \end{subfigure}\\ &&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{truck:$0.32$, $p:1.00$, $p_R:0.99$, $p_{NR}:0.93$, $p_{RA}:1.00$, $MSE: 0.58$, $MSE_c: 1.08$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_20_from_truck_to_truck_start=0.32414,end=0.99978_l_0_3070.0,l_1_34.89,l_2_1.05,l_inf_0.16,LPIPS_0.23_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{truck:$0.44$, $p:1.00$, $p_R:0.99$, $p_{NR}:0.94$, $p_{RA}:1.00$, $MSE: 0.61$, $MSE_c: 1.36$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_20_from_truck_to_truck_start=0.43986,end=0.99976_l_0_3070.0,l_1_28.77,l_2_0.89,l_inf_0.15,LPIPS_0.21_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{truck:$0.43$, $p:1.00$, $p_R:0.98$, $p_{NR}:0.95$, $p_{RA}:1.00$, $MSE: 0.61$, $MSE_c: 1.16$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_20_from_truck_to_truck_start=0.43145,end=0.99976_l_0_3070.0,l_1_26.55,l_2_0.78,l_inf_0.14,LPIPS_0.18_last.png}
                
                \end{subfigure}\\& \begin{subfigure}{0.12\textwidth}\centering
     \vspace*{26.8mm}
     \caption*{deer/cat}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/init_56_from_cat_to_deer_start=0.40394,end=0.99974_l_0_3072.0,l_1_25.41,l_2_0.82,l_inf_0.10,LPIPS_0.40_first.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{deer:$0.32$, $p:1.00$, $p_R:0.99$, $p_{NR}:0.96$, $p_{RA}:0.93$, $MSE: 2.79$, $MSE_c: 1.54$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_56_from_cat_to_deer_start=0.31946,end=0.99974_l_0_3072.0,l_1_57.46,l_2_1.63,l_inf_0.16,LPIPS_0.50_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{deer:$0.47$, $p:1.00$, $p_R:0.97$, $p_{NR}:0.96$, $p_{RA}:0.49$, $MSE: 3.22$, $MSE_c: 1.68$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_56_from_cat_to_deer_start=0.46590,end=0.99975_l_0_3072.0,l_1_34.46,l_2_1.05,l_inf_0.13,LPIPS_0.44_last.png}
     
     \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
     
     \caption*{deer:$0.40$, $p:1.00$, $p_R:0.96$, $p_{NR}:0.96$, $p_{RA}:0.27$, $MSE: 3.22$, $MSE_c: 1.77$}
     \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_56_from_cat_to_deer_start=0.40394,end=0.99974_l_0_3072.0,l_1_25.41,l_2_0.82,l_inf_0.10,LPIPS_0.40_last.png}
     
     \end{subfigure}\\ &&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{cat:$0.45$, $p:1.00$, $p_R:0.79$, $p_{NR}:0.02$, $p_{RA}:0.15$, $MSE: 3.17$, $MSE_c: 4.36$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.25eps_56_from_cat_to_cat_start=0.45226,end=0.99975_l_0_3072.0,l_1_76.05,l_2_2.02,l_inf_0.20,LPIPS_0.60_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{cat:$0.36$, $p:1.00$, $p_R:0.62$, $p_{NR}:0.10$, $p_{RA}:0.13$, $MSE: 3.46$, $MSE_c: 4.47$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.1eps_56_from_cat_to_cat_start=0.35810,end=0.99974_l_0_3072.0,l_1_57.65,l_2_1.48,l_inf_0.13,LPIPS_0.59_last.png}
                
                \end{subfigure}&\begin{subfigure}{0.12\textwidth}\centering
                
                \caption*{cat:$0.43$, $p:1.00$, $p_R:0.36$, $p_{NR}:0.02$, $p_{RA}:0.13$, $MSE: 3.49$, $MSE_c: 4.62$}
                \includegraphics[width=1\textwidth]{inverse_smaller_radius_latex_images/0.02eps_56_from_cat_to_cat_start=0.43231,end=0.99975_l_0_3072.0,l_1_38.26,l_2_1.07,l_inf_0.11,LPIPS_0.55_last.png}
                
                \end{subfigure}\\
     \hline
     \end{tabular}
     \end{adjustbox}
     \caption{\label{tab:Inverse_poblem}Counterfactuals of different models using PGD for a fixed radius of the $l^2$ ball $\epsilon=2.5$.}
     \end{table*}
            

==> panels/watermark_confidence.tex <==

\begin{figure}[hbt!]
     \begin{adjustbox}{width=1\columnwidth,center}
     \centering
     \begin{tabular}{cc}
     \begin{subfigure}{0.5\textwidth}\centering
     
     
     \includegraphics[width=1\textwidth]{images/spurious_features/Watermark_conf.pdf}
     \end{subfigure}&\begin{subfigure}{0.3\textwidth}\centering
     \vspace*{-3mm}
     \includegraphics[width=1\textwidth]{images/spurious_features/istockphoto_max_confidence.png}
     \caption*{$p_e$:$0.98$, intensity:$0.5$}

     
     \end{subfigure}\\
     \end{tabular}
     \end{adjustbox}
     \caption{\label{fig:varying_intensity}On the left the end probability vs. intensity is displayed. On the right - the augmented image with the highest end confidence.}
     \end{figure}


